PolarBEVDet: Exploring Polar Representation for Multi-View 3D Object Detection in Bird's-Eye-View

Recently, LSS-based multi-view 3D object detection provides an economical and deployment-friendly solution for autonomous driving. However, all the existing LSS-based methods transform multi-view image features into a Cartesian Bird's-Eye-View(BEV) representation, which does not take into account the non-uniform image information distribution and hardly exploits the view symmetry. In this paper, in order to adapt the image information distribution and preserve the view symmetry by regular convolution, we propose to employ the polar BEV representation to substitute the Cartesian BEV representation. To achieve this, we elaborately tailor three modules: a polar view transformer to generate the polar BEV representation, a polar temporal fusion module for fusing historical polar BEV features and a polar detection head to predict the polar-parameterized representation of the object. In addition, we design a 2D auxiliary detection head and a spatial attention enhancement module to improve the quality of feature extraction in perspective view and BEV, respectively. Finally, we integrate the above improvements into a novel multi-view 3D object detector, PolarBEVDet. Experiments on nuScenes show that PolarBEVDet achieves the superior performance. The code is available at https://github.com/Yzichen/PolarBEVDet.git.(This work has been submitted to the IEEE for possible publication. Copyright may be transferred without notice, after which this version may no longer be accessible)

==> sections/author.tex <==
\vskip 0pt plus -1fil
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip]{figures/author/yzc.pdf}}]{Zichen Yu}
    received the B.S. degree from Harbin Engineering University, Harbin, China in 2018 and the M.S degree 
    from Dalian University of Technology, Dalian, China in 2020, where he is currently pursuing the Ph.D. 
    in control theory and engineering.
    His research interests include lane detection and 3D object detection.
\end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip]{figures/author/lql.pdf}}]{Quanli Liu}
    (Member, IEEE) received the B.Sc. and M.Sc. degrees in control theory and engineering from Northeastern
    University, Shenyang, China, in 1998 and 2000, respectively, and received the Ph.D. degree in automation
    from Dalian University of Technology, Dalian, China, in 2005. He is currently a Professor at Dalian
    University of Technology. 
    His research interests include production planning and scheduling, industrial process control, computer vision, 
    machine learning and discrete event simulation.
\end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip]{figures/author/ww.pdf}}]{Wei Wang}
    (Senior Member, IEEE) received the B.S., M.S., and Ph.D. degrees from Northeastern University, Shenyang, China, 
    in 1982, 1986, and 1988, respectively, all in industrial automation. He was a Postdoctoral Fellow with the Division
    of Engineering Cybernetics, Norwegian Science and Technology University, Trondheim, Norway, from 1990 to 1992, a Professor 
    and the Vice Director of the National Engineering Research Center of Metallurgical Automation of China, Shenyang, from 1995 to 1999, 
    and a Research Fellow with the Department of Engineering Science, University of Oxford, Oxford, U.K., from 1998 to 1999. 
    He is currently a Professor with the School of Control Sciences and Engineering, Dalian University of Technology, Dalian, China. 
    His current research interests include adaptive controls, computer-integrated manufacturing, and computer controls of industrial processes.
\end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip]{figures/author/zly.pdf}}]{Liyong Zhang}
    (Member, IEEE) received the B.S. degree in Automation, the M.S. degree in Control Theory and Control Engineering and the Ph.D. degree 
    in Control Theory and Control Engineering from Dalian University of Technology, Dalian, China, in 1999, 2002 and 2018, respectively. 
    He is currently working as an Associate Professor in the School of Control Science and Engineering, Dalian University of Technology. 
    He has published more than 80 research papers, has 5 Chinese invention patents issued, and is a coauthor of 3 books. His current 
    research interests include data modeling, fuzzy clustering, granular computing, and equipment Intelligence. He also serves as a 
    Reviewer for many international journals including IEEE Transactions on Cybernetics, IEEE Transactions on Systems, Man and 
    Cybernetics: Systems, IEEE Transactions on Fuzzy Systems, Neurocomputing, Applied Soft Computing, Knowledge-Based Systems, 
    Softcomputing, Applied Intelligence.
\end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip]{figures/author/zxg.pdf}}]{Xiaoguang Zhao}
    received the B.S. and M.S. degrees from Dalian University of Technology, Dalian, China, in 2007 and 2010, respectively. 
    Since 2010, he has been working with Dalian Seasky Automation Company, Ltd., Dalian. 
    His research interests include embedded system design, accelerated computing, machine learning, and compute vision application.
\end{IEEEbiography}

